Gazelle: An Instruction Dataset for Arabic Writing Assistance

Writing has long been considered a hallmark of human intelligence and remains a pinnacle task for artificial intelligence (AI) due to the intricate cognitive processes involved. Recently, rapid advancements in generative AI, particularly through the development of Large Language Models (LLMs), have significantly transformed the landscape of writing assistance. However, underrepresented languages like Arabic encounter significant challenges in the development of advanced AI writing tools, largely due to the limited availability of data. This scarcity constrains the training of effective models, impeding the creation of sophisticated writing assistance technologies. To address these issues, we present Gazelle, a comprehensive dataset for Arabic writing assistance. In addition, we offer an evaluation framework designed to enhance Arabic writing assistance tools. Our human evaluation of leading LLMs, including GPT-4, GPT-4o, Cohere Command R+, and Gemini 1.5 Pro, highlights their respective strengths and limitations in addressing the challenges of Arabic writing. Our findings underscore the need for continuous model training and dataset enrichment to manage the complexities of Arabic language processing, paving the way for more effective AI-powered Arabic writing tools.

==> Tables/Data_Stats.tex <==
\begin{table}[t]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lccccc}
\toprule
\textbf{Task} & \textbf{Language / Category} & \textbf{Total} & \textbf{Train} & \textbf{Test} \\
\midrule
\multirow{2}{*}{\textbf{Explanation and Definitions}} & \hl{Arabic -websites} & 1445 & 1395 & 50 \\
 & \hl{English- websites} & 1005 & 955 & 50 \\
\midrule
\multirow{2}{*}{\textbf{Metaphors}} & \hl{Arabic -books} & 230 & 180 & 50 \\
 & \hl{English- translated}  & 230 & 180 & 50 \\
\midrule
\multirow{2}{*}{\textbf{MWE}} & \hl{Arabic- PARSEM dataset} & 98 & 68 & 30 \\
 & \hl{English- translated} & 98 & 68 & 30 \\
\midrule
\multirow{2}{*}{\textbf{Text Upscaling}} & \hl{Arabic- an in-house project dataset} & 770 & 720 & 50 \\
 & \hl{English-translated} & 770 & 720 & 50 \\
\midrule
\textbf{Irab} & \hl{Arabic- websites + books} & 1090 & 1040 & 50 \\
\midrule
\multirow{5}{*}{\textbf{GEC}} & \hl{Orthographic- websites+books} & 637 & - & - \\
 & \hl{Syntax-websites+books} & 377 & - & - \\
 & \hl{Semantic-websites+books} & 362 & - & - \\
 & \hl{Morphology-websites+books} & 55 & - & - \\
 & \hl{Punctuation-websites} & 28 & - & - \\
\midrule
\textbf{GEC\_ATB} & Arabic & 1433 & - & - \\
\textbf{GEC + Definition} & Arabic &  & - & - \\
    \textbf{GEC + Explanation} & Arabic &  & - & - \\
\bottomrule
\end{tabular}%
}
\caption{Data statistics for various tasks with language and category differentiation.}
\label{data_stats}
\end{table}


==> Tables/comparison_final.tex <==
\begin{table*}[]
\resizebox{\textwidth}{!}{%
\begin{tabular}{cllclcrr}
\toprule
\multicolumn{7}{c}{\textbf{Gazelle Dataset}}                                                                                                                                                                 \\ \midrule
\multicolumn{2}{c}{\colorbox{gray!10}{\textbf{QALB}}}                    &          & \multicolumn{2}{c}{\colorbox{green!10}{\textbf{New tasks}}} & & \multicolumn{2}{c}{\textbf{Examples}}                                                                                                                                                                                                  \\ \cmidrule{1-2} \cmidrule{4-5} \cmidrule{7-8}
\colorbox{gray!10}{\textbf{Type} }                 & \colorbox{gray!10}{\textbf{Tag}}       &                    & \colorbox{green!10}{\textbf{Subclass}}                                 & \multicolumn{1}{c}{\colorbox{green!10}{\textbf{Sub2}}}       &  & \multicolumn{1}{c}{\textbf{Wrong}}                                    & \multicolumn{1}{c}{\textbf{Correct}}                                 \\ \midrule

                                        &                                              &                 & & Medial Hamza                    & &
                                        \n \AR{كانت تلك} \r\AR{مسالة} \n \AR{هامة.}
                                        &    \n \AR{كانت تلك} \g\AR{مسألة} \n \AR{هامة.}                                             \\
                                        &                                              &                                                      &   & Hamzet Wasel                &    & \n \AR{إستبشرت} \r\AR{بالمطر خيراً.}              & \n \AR{استبشرت} \g\AR{بالمطر خيراً.}                           \\
                                        &                                              &                                                     &    & The Cutting Hamzah             & & \n \AR{بخصوص تأمين سكن وظيفي في} \r\AR{احد} \n \AR{السكنات.}              & \n \AR{بخصوص تأمين سكن وظيفي في} \g\AR{أحد} \n \AR{السكنات.}          \\
\multirow{-4}{*}{\rotatebox[origin=c]{90}{\textbf{Orth.}}} & \multirow{-3}{*}{OH}                       &  & \multirow{-4}{*}{Hamza}                                 & Final Hamza    &                 & \n \AR{لا} \r\AR{يجروء} \n \AR{المسلم على الكذب.}           & \n \AR{لا} \g\AR{يجرؤ} \n \AR{المسلم على الكذب.}                     \\ \midrule
                                        &                                              &                           &                              & Masculine Sound Plural       &   & \n\AR{سائقوا} \r\AR{السيارات ملتزمون بتعليمات إدارة المرور.}& \n\AR{سائقو} \g\AR{السيارات ملتزمون بتعليمات إدارة المرور.} \\ 
                                        &                      &                        & \multirow{-2}{*}{Plural}                                & Almaqsour Plural              &  & \n\AR{وعلى مرمى طوبة زمن منا ونحن لا نعيه،} \r\AR{بُلَهَاء} \n\AR{لا ندركه.} &  \n\AR{وعلى مرمى طوبة زمن منا ونحن لا نعيه،} \g\AR{بُلْهٌ} \n\AR{لا ندركه.} \\\cmidrule{4-8}
                                        &               &                               &                                                         & Composite Numbers            &  &\r\AR{عشر}\n\AR{يمكنكم الآن مشاهدة الحلقة الثالثة} & \g\AR{عشرة}\n\AR{يمكنكم الآن مشاهدة الحلقة الثالثة}  \\
\multirow{-4}{*}{\rotatebox[origin=c]{90}{\textbf{Syntax}}}       & \multirow{-4}{*}{XN}            &             & \multirow{-2}{*}{Number}                                & Al Aqoud                   &  & \n\AR{حضر مريض في} \r\AR{الخمسون} \n\AR{من عمره.} &  \n\AR{حضر مريض في} \g\AR{الخمسين} \n\AR{من عمره.} \\ \midrule
                                        & \multirow{4}{*}{SW}            &             & \multirow{4}{*}{Word Selection Error}                                & Adding Unnecessary Prepositions                   &  & \n\AR{تحرى فلان} \r\AR{عن} \n\AR{الأمر.} &  \n\AR{تحرى فلان} \g\AR{الأمر.} \\ \cmidrule{5-8}

                                        &               &                               &                                                         & Removing Necessary Prepositions             &  &\n\AR{تسعى الدولة} \r\AR{تحقيق} \n\AR{مكاسب دولية.} & \n\AR{تسعى الدولة} \g\AR{إلى تحقيق} \n\AR{مكاسب دولية.}  \\ \cmidrule{5-8}

                                        &               &                               &                                                         & Replacing Prepositions             &  &\r\AR{في}\n\AR{ثم وجدت طلبا} \r\AR{في} \n\AR{بلاد مختلفة.} & \g\AR{من} \n\AR{ثم وجدت طلبا} \g\AR{من} \n\AR{بلاد مختلفة.} \\ \midrule

\multirow{-3}{*}{\rotatebox[origin=c]{90}{\textbf{Semantics}}}       & \multirow{3}{*}{SF}            &             & \multirow{3}{*}{Conjunction Error}                                & Adding Unnecessary Conjunction                   &  & \n\AR{ووصلت صدى هذه الأصوات} \r\AR{حتى} \n\AR{إلى قلوب بعض المسلمين والمسلمات.} & \n\AR{ووصلت صدى هذه الأصوات} \g\AR{إلى} \n\AR{قلوب بعض المسلمين والمسلمات.} \\ \cmidrule{5-8}
                                            &               &                               &                                                         & Removing Necessary Conjunction             &  &\r\AR{و}\n\AR{اذهب إلى فلان} \r\AR{وقل له كذا.} & \g\AR{فقل} \n\AR{اذهب إلى فلان} \g\AR{فقل له كذا.}  \\ \midrule

\multirow{-4}{*}{\rotatebox[origin=c]{90}{\textbf{Punctuation}}}       & \multirow{1}{*}{PO}            &             & Other Punctuation                               &            &  & \r\AR{مرحباً} \n\AR{كيف حالك.} & \g\AR{مرحباً،} \n\AR{كيف حالك؟}  \\ \cmidrule{2-8}
                                            & \multirow{1}{*}{PC}            &             & Punctuation Confusion                               &            &  & \r\AR{أحب القراءة،} \n\AR{والكتابة.} & \g\AR{أحب القراءة والكتابة.}  \\ \cmidrule{2-8}
                                            & \multirow{1}{*}{PM}            &             & Punctuation Missing                               &            &  & \r\AR{هل يستطيع هذا القس أن يعلن} \n\AR{رغبته.} & \g\AR{هل يستطيع هذا القس أن يعلن} \g\AR{رغبته؟}  \\ \cmidrule{2-8}                                                                                         
\end{tabular}%
}
\caption{Add caption here.....}
\label{comparsion}
\end{table*}


==> Tables/figure3.tex <==
\begin{table*}[!htp]\centering
\centering
\scriptsize % Slightly reduce font size to make table narrower
\resizebox{\textwidth}{!}{%
\begin{tabular}{l p{2.5cm} p{2cm} p{2cm} p{3.5cm} p{3.5cm} p{5cm}} % Adjust column widths
\toprule
\rowcolor{gray!20} % Add row color here
\textbf{Task} & \textbf{Error Class} & \textbf{Error Sub-Class} & \textbf{Error Sub-subclass} &  \textbf{Incorrect Sentence} & \textbf{Corrected Sentence} & \textbf{Explanation} \\
\midrule
 \cellcolor{cyan!20}& \textbf{Morphology} & \textbf{Verb Tense} & - & \AR{سجلت وحدات الحماية المدنية 999. حادث مرور أدت إلى وفاة 32 شخصا.} & \AR{سجلت وحدات الحماية المدنية 999. حادث مرور أدى إلى وفاة 32 شخصا.} & \AR{الخطأ في الفعل أدى، يعبر عن حدث أو موقف مذكر لذلك يجب أن يكون خالي من تاء التأنيث.} \\
  \cellcolor{cyan!20}& \textbf{Orthography} & \textbf{Final Hamza} & - & \AR{هذا الصبي بطِي في الجري.} & \AR{هذا الصبي بطِيء في الجري.} & \AR{الخطأ في كلمة بطيء: كتبت الهمزة المتطرفة على الياء لأن حركة الحرف الذي قبلها الكسرة.} \\
  \cellcolor{cyan!20}& \textbf{Punctuation} & \textbf{Comma} & - & \AR{قال محمود درويش، أحنُّ إلى خبز أمي وقهوة أُمي.} & \AR{قال محمود درويش: أحنُّ إلى خبز أمي وقهوة أُمي.} & \AR{الخطأ هو الفاصلة (،)؛ لأنها تستخدم لفصل الجمل المترابطة، والصحيح يجب أن تكون نقطتان رأسيتان (:)؛ لأنها تأتي بعد القول.} \\
  \cellcolor{cyan!20} \multirow{7}{*}{\centering \textbf{GEC}}& \textbf{Semantic} & \textbf{Conjugation Error} & \textbf{Removing unnecessary conjugation} & \AR{سفير دمشق بلندن: قرينة الرئيس لم لن تغادر دمشق.} & \AR{سفير دمشق بلندن: قرينة الرئيس لم ولن تغادر دمشق.} & \AR{الخطأ في حذف حرف العطف الواو بين كلمتي لم ولن في الجملة حيث أتت عطف الواو بين أداتي نفي مختلفتين في العمل إحدهما جازمة والأخرى ناصبة.} \\
  \cellcolor{cyan!20}& \textbf{Syntax} & \textbf{Definiteness} & \textbf{Adding "AI"} & \AR{رأيت أول المسجد في الإسلام.} & \AR{رأيت أول مسجد في الإسلام.} & \AR{الخطأ: زيادة “ال” التعريف على المضاف لأنه لا يجب أن يكون المضاف والمضاف إليه مشتركين في التعريف والتنكير.} \\
  \cellcolor{cyan!20}& \textbf{Split} & - & - & \AR{اتحاد العاب القوى يكرم الا بطال.} & \AR{اتحاد العاب القوى يكرم الابطال.} & \AR{الخطأ في هذه الكلمة: الا بطال حيث يفترض أن تكون: الابطال} \\
  \cellcolor{cyan!20}& \textbf{Merge} & - & - & \AR{ونفتتقارير عن أن مدنيين قتلوا في الهجوم الجوي.} & \AR{ونفت تقارير عن أن مدنيين قتلوا في الهجوم الجوي.} & \AR{الخطأ في هذه الكلمة: ونفتتقارير حيث يفترض أن تكون: ونفت تقارير} \\
\midrule
 \cellcolor{orange!20}\textbf{Metaphors}& \AR{التشبيه} & - & - & \AR{كان نقده كالملح في العسل.} & \AR{كان نقده كالسم في العسل.} & \AR{الخطأ في استخدام التعبير كالملح في العسل، مما يغير المعنى المقصود من شيء ضار متنكر كشيء حلو إلى شيء غير متناسب ولكنه أقل ضررًا.} \\
\midrule
 \cellcolor{green!20}\textbf{Multi-Words Expression}& \AR{التعبيرات المتعددة} & - & - & \AR{وقد لمح بذلك إلى قيادة “الموساد المخابرات الإسرائيلية التي تريد أن تأخذ على رأسها مسؤولية الحملة الدولية إيران باعتباره موضوعاً أمنيا.} & \AR{وقد لمح بذلك إلى قيادة الموساد المخابرات الإسرائيلية التي تريد أن تأخذ على عاتقها مسؤولية الحملة الدولية ضد إيران باعتباره موضوعاً أمنيا.} & \AR{الخطأ في استخدام التعبير تأخذ على رأسها مما يغير المعنى المقصود من تحمل المسؤولية إلى شيء غير منطقي.} \\
\midrule
 \cellcolor{red!20}\textbf{Text Up-Scaling}& \AR{تحويل الأسلوب} & - & - & \AR{وأنت تعرف جيداً، ولا عارف أن أصابعنا تحت ضرسه.} & \AR{وأنت تعرف جيدًا، وتعرف أن حياتنا بين يديه.} & \AR{(أصابعنا تحت ضرسه) مصطلح مصري عامي بمعنى أنهم تحت رحمته أو تحكمه، ولا يصح كتابته في الفصحى.} \\
\bottomrule
\end{tabular}%
}
\caption{Examples from five different writing tasks, including incorrect sentences, their corrected versions, and detailed explanations of the errors and corrections. The tasks encompass \textit{Grammatical Error Correction} (GEC), \textit{Grammatical Error Explanation}, \textit{Metaphors and Multi-word Expressions} (MWEs), and \textit{Text Up-scaling}.}
\label{tab:error_comparison}
\end{table*}


==> Tables/wrong_correct.tex <==
\begin{table*}[h]
\centering


\renewcommand{\arraystretch}{1.0}   %to squeeze table content low value means squeeze more
\resizebox{1.\linewidth}{!}{% reduce the text size, lower 
\begin{tabular}{lllrrr}
\toprule
\textbf{Error Class} & \textbf{Error SubClass} & \textbf{Error Sub-subclass}& 
\multicolumn{1}{c}{\textbf{Wrong}} 
&    \multicolumn{1}{c}{\textbf{Correct}}  &  \multicolumn{1}{c}{\textbf{Explanation}} \\ \midrule
Morphology & Verb Tense & - & \begin{tabular}{r}
            {\large \<سجلت وحدات الحماية المدنية 999.>} \\
             {\large \<حادث مرور أدت إلى وفاة 32 شخصا.>} \\
        \end{tabular}            & \begin{tabular}{r}
            {\large \<سجلت وحدات الحماية المدنية 999. >}\\
            {\large \<حادث مرور أدى إلى وفاة 32 شخصا.>} \\
        \end{tabular} & \begin{tabular}{r}
            {\large \< الخطاء في الفعل أدى،>} \\
            {\large \< يعبر عن حدث أو موقف مذكر > } \\
            {\large \<لذلك يجب أن يكون خالي من تاء التأنيث. >}
        \end{tabular} \\ 
Orthography & Final Hamza & - & \begin{tabular}{r}
            {\large \<هذا الصبي بطِي في الجري.>} \\
        \end{tabular}        & \begin{tabular}{r}
            {\large \< هذا الصبي بطِيء في الجري.>}\\
        \end{tabular} & \begin{tabular}{r}
            {\large \<الخطاء في كلمة بطيء: كتبت الهمزة المتطرفة>} \\
            {\large \<على الياء لأن حركة الحرف الذي قبلها الكسرة. > } \\
        \end{tabular} \\ &  \\
Punctuation & Comma & - & \begin{tabular}{r}
            {\large \<قال محمود درويش،>} \\
            {\large \<أحنُّ إلى خبز أمي وقهوة أُمي.>}\\
        \end{tabular}& \begin{tabular}{r}
            {\large \<قال محمود درويش: >}\\
            {\large \<أحنُّ إلى خبز أمي وقهوة أُمي.>}\\
        \end{tabular} & \begin{tabular}{r}
            {\large \<الخطأ هو الفاصلة (،)؛ >} \\
            {\large \< لأنها تستخدم لفصل الجمل المترابطة،>} \\
            {\large \< والصحيح يجب أن تكون نقطتان؛> } \\
            {\large \< رأسيتان (:)؛ لأنها تأتي بعد القول.>}
        \end{tabular} \\ &  \\&  \\
Semantics & Conjunction Error & Removing Necessary Conjunction & \begin{tabular}{r}
            {\large \<سفير دمشق بلندن:>} \\
            {\large \< قرينة الرئيس لم لن تغادر دمشق.>}\\
        \end{tabular} & \begin{tabular}{r}
            {\large \< سفير دمشق بلندن:>}\\
             {\large \< قرينة الرئيس لم ولن تغادر دمشق.>}\\
        \end{tabular} & \begin{tabular}{r}
            {\large \<الخطأ في حذف حرف العطف الواو >} \\
            {\large \< بين كلمتي لم ولن في الجملة>} \\
            {\large \<   حيث أتت عطف الواو بين أداتي> } \\
            {\large \<نفي مختلفتين في العمل إحدهما جازمة والأخرى ناصبة. >}
            {\large \<  >} \\
        \end{tabular} \\& \\
Syntax & Definiteness & Adding "Al" & \begin{tabular}{r}
            {\large \<رأيت أول المسجد في الإسلام.>} \\
        \end{tabular} &\begin{tabular}{r}
            {\large \<رأيت أول مسجد في الإسلام.>} \\
        \end{tabular} & \begin{tabular}{r}
            {\large \<الخطاء: زيادة "ال" التعريف على المضاف >}\\
            {\large \< لانه لايجب أن المضاف والمضاف إليه >} \\
            {\large \<أن يكونا مشتركين في التعريف والتنكير.>}\\
        \end{tabular}&
% Add more rows as needed

Metaphors & - & - & \begin{tabular}{r}
            {\large \<كان نقده كالملح في العسل.>} \\
        \end{tabular} &\begin{tabular}{r}
            {\large \<كان نقده كالسم في العسل.>} \\
        \end{tabular} & \begin{tabular}{r}
            {\large \<الخطأ في استخدام التعبير كالملح في العسل،>}\\
            {\large \< مما يغير المعنى المقصود من شيء ضار متنكر >} \\
            {\large \< كشيء حلو إلى شيء غير متناسب ولكنه أقل ضررًا.>}\\
        \end{tabular}&
MWEs & - & - & \begin{tabular}{r}
            {\large \<وقد لمح بذلك إلى قيادة "الموساد المخابرات>} \\
             {\large \<الإسرائيلية التي تريد أن تأخذ على رأسها>} \\
             {\large \<مسؤولية الحملة الدولية >} \\
              {\large \<إيران باعتباره موضوعاً أمنيا. >} \\
        \end{tabular} &\begin{tabular}{r}
            {\large \<وقد لمح بذلك إلى قيادة الموساد المخابرات>} \\
             {\large \<الإسرائيلية التي تريد أن تأخذ على عاتقها>} \\
              {\large \<مسؤولية الحملة الدولية ضد >} \\
              {\large \<إيران باعتباره موضوعاً أمنيا. >} \\
        \end{tabular} & \begin{tabular}{r}
            {\large \<الخطأ في استخدام التعبير تأخذ على رأسها >}\\
            {\large \< مما يغير المعنى المقصود من >} \\
            {\large \< تحمل المسؤولية إلى شيء غير منطقي.>}\\
        \end{tabular}&
Style Transfer & - & - & \begin{tabular}{r}
            {\large \<وأنت تعرف جيداً،>} \\
             {\large \<ولا عارف أن أصابعنا تحت ضرسه. >} \\
        \end{tabular} &\begin{tabular}{r}
            {\large \<وأنت تعرف جيدًا،>} \\
             {\large \<وتعرف أن حياتنا بين يديه.>} \\
        \end{tabular} & \begin{tabular}{r}
            {\large \<(أصابعنا تحت ضرسه) مصطلح مصري>}\\
            {\large \< عامي بمعنى أنهم تحت رحمته أو تحكمه،>} \\
            {\large \<ولا يصح كتابته في الفصحى.>}\\
        \end{tabular}&
Split & - & - & \begin{tabular}{r}
            {\large \<اتحاد العاب القوى يكرم الا بطال >} \\
        \end{tabular} &\begin{tabular}{r}
            {\large \<اتحاد العاب القوى يكرم الابطال>} \\  
        \end{tabular} & \begin{tabular}{r}
            {\large \< الخطأ في هذه الكلمة: الا بطال >}\\
            {\large \<حيث يفترض أن تكون: الابطال >} \\
        \end{tabular}&        
Merge & - & - & \begin{tabular}{r}
            {\large \<ونفتتقارير عن أن مدنيين >} \\
             {\large \< .قتلوا في الهجوم الجوي>} \\
        \end{tabular} &\begin{tabular}{r}
            {\large \<ونفت تقارير عن أن مدنيين >} \\
             {\large \<قتلوا في الهجوم الجوي>} \\
        \end{tabular} & \begin{tabular}{r}
            {\large \< الخطأ في هذه الكلمة: ونفتتقارير  >}\\
            {\large \< حيث يفترض أن تكون: ونفت تقارير >} \\
        \end{tabular}&     
\end{tabular}
} \\ \bottomrule

\vspace{1em}
\caption{\label{Examples of the wrong and correct forms of the sentences along with the explanation of errors}
Examples of the wrong and correct forms of the sentences along with the explanations of the errors
}
\label{tab:Table1}

\end{table*}
